Simultaneous approximation of a smooth function and its derivatives by deep neural networks with piecewise-polynomial activations

This paper investigates the approximation properties of deep neural networks with piecewise-polynomial activation functions. We derive the required depth, width, and sparsity of a deep neural network to approximate any H\"{o}lder smooth function up to a given approximation error in H\"{o}lder norms in such a way that all weights of this neural network are bounded by $1$. The latter feature is essential to control generalization errors in many statistical and machine learning applications.

==> lit_review.tex <==
Literature on approximation properties of neural networks with RePU activations.
\begin{itemize}
    %\item \cite{li20a} -- the same results as in \cite{li20b}.
    \item \cite{li20b} -- exact representation of polynomials via RePU neural networks, optimal rates of approximation of smooth functions (from Jacobi-weighted Sobolev space) with respect to a weighted $L_2$-norm.
    \item \cite{ozawa19}
    %\item \cite{siegel19} -- approximation of a smooth function with respect to the Sobolev norm $H^m([0,1]^d)$, non-standard smoothness class, strange rates of approximation, shallow neural networks (two layers).
    \item \cite{ali21} -- $f \in B^\alpha_\tau(L_\tau(\Omega))$, $\Omega$ is an $(\eps, \delta)$-domain or a Lipschitz domain, approximation in $L_p(\Omega)$-norm, $\alpha \geq 1/\tau + 1/p$, RePU and ReLU neural networks, approximation rate $\alpha/d$ for RePU (for ReLU the same rate up to log-factors).
    \item \cite{gribonval22} -- $f \in B^\alpha_p(L_p(\Omega))$, $\alpha < 1/d + \min\{1, 1/p\}$, $\Omega$ is a bounded Lipschitz domain, approximation in $L_p(\Omega)$-norm, RePU neural networks, approximation rate $\alpha/d$.
    \item \cite{mhaskar93} 
    \item \cite{hon21} -- \red{check the result}, approximation of $f$ w.r.t. the $W^{1, p}([0,1]^d)$-norm via ReLU neural networks and w.r.t. the $W^{k, p}([0,1]^d)$-norm, $k > 1$, via ReQU neural networks. An explicit and user-friendly bound on the approximation error. No bounds on the absolute value of the weights. No bounds on the number of active neurons. Requires different neural networks for different values of $k$. Submitted to Neural Networks on 24 January, 2022.
    \item \cite{abdeljawad22} -- approximation in Sobolev norm for $f: \rset^{d+1} \mapsto \rset$ in $W^{k, p}_{r,q}([0,1] \times [0,1]^d)$ norm. $1$-st component has different regularity (time and space structure, adopted f PDEs). Uses ReCU activations (cubic). Same drawbacks as \cite{guhring21}: weights and width of order $\eps^{-\theta}$.
    \item \cite{klusowski18} -- approximation via neural networks with ReQU activations and one hidden layer with respect to the $L_\infty$-norm, the smoothness of a target function is described in terms of its Fourier transform.
    \item \cite{chen22} -- PSENet (power series expansion neural network); has one hidden layer with activations $\sigma(x), \sigma^2(x), \dots, \sigma^n(x)$. Upper bound on the $W^{m, 2}$-norm of the error in one-dimensional case. Upper bound on the approximation error for polynomials in the multidimensional case.
\end{itemize}

Approximation with respect to H\"{o}lder and Sobolev norms.
\begin{itemize}
    \item \cite{guhring20}
    \item \cite{guhring21} -- the closest result to ours, but no results on the H\"older norm of the approximation itself. The architecture of DNN depends on the smoothness of the function. The weights are bounded in absolute value by $\eps^{-\theta}$ where $\theta $ depends on the norm. This yields the covering number issues discussed in \Cref{sec:applications}. \red{N. P.: we have no such section.} 
    \item \cite{deryck21} -- slightly improves over \cite{guhring21}, but is based on a very similar to \cite{guhring21} technique and, as consequence, inherits the drawbacks of \cite{guhring21}, discussed above.
    \item \cite{dung21} -- \red{check the result}, approximation of an $\alpha$-smooth function from a H\"{o}lder-Zygmund space (vanishing at the boundary of $[0, 1]^d$) with respect to the $W^{1, p}_0$-norm, ReLU activations, the width of the neural network scales as $\eps^{-1/(\alpha-1)} \log(1/\eps)$, instead of $\eps^{-d/(\alpha-1)}$; Theorem 4.1 is strange and leads to the rates of estimation contradicting with the existing lower bounds.
\end{itemize}

Approximation with respect to the $L_p$-norm.
\begin{itemize}
    \item \cite{yarotsky17}
    \item \cite{langer21} -- $f$ is $(p, C)$-smooth, approximation in $L_\infty$-norm, sigmoid activations, neural networks of fixed depth, fully-connected neural networks, the widths of all the layers are the same, approximation rate $p/d$, approximation on a cube $[-a, a]^d$ but $f$ must be smoothly continued to $[-2a, 2a]^d$. 
    \item \cite{suzuki19}
    \item \cite{lu21} -- approximating $f \in C^{s}([0,1]^{d})$ by ReLU deep NN in $L_{\infty}$-norm. 
    \item \cite{jiao21} - approximating $f \in \H^{\alpha}([0,1]^d)$ in $L_p$-norm, $p \in [1;+\infty]$. Architecture: constant depth $(L=6)$, mixed activations (ReLU, sinus, $2^{x}$).
    \item \cite{shen20} -- $f \in \H^{\alpha}([0,1]^d)$, approximation w.r.t. the $L_p$-norm; approximation of smooth functions on $\eps$-neighborhoods of low-dimensional manifolds.
    \item \cite{shen21} -- approximating continuous functions in $L_p$-norm, bounds in terms of modulus of continuity. Constant depth, activations: floor ($\lfloor \cdot \rfloor$), exponential, indicator.
    \item \cite{montanelli19}
    \item \cite{yarotsky18}
    \item \cite{yarotsky20}
\end{itemize}
